Finding accreted stars in the Milky Way: clues from NIHAO simulations

Exploring the marks left by galactic accretion in the Milky Way helps us understand how our Galaxy was formed. However, finding and studying accreted stars and the galaxies they came from has been challenging. This study uses a simulation from the NIHAO project, which now includes a wider range of chemical compositions, to find better ways to spot these accreted stars. By comparing our findings with data from the GALAH spectroscopic survey, we confirm that the observationally established diagnostics of [Al/Fe] vs. [Mg/Mn] also show a separation of in-situ and accreted stars in the simulation, but stars from different accretion events tend to overlap in this plane even without observational uncertainties. Looking at the relationship between stellar age and linear or logarithmic abundances, such as [Fe/H], we can clearly separate different groups of these stars if the uncertainties in their chemical makeup are less than 0.15 dex and less than 20% for their ages. This method shows promise for studying the history of the Milky Way and other galaxies. Our work highlights how important it is to have accurate measurements of stellar ages and chemical content. It also shows how simulations can help us understand the complex process of galaxies merging and suggest how these events might relate to the differences we see between our Galaxy's thin and thick disk stars. This study provides a way to compare theoretical models with real observations, opening new paths for research in both our own Galaxy and beyond.

==> tex_text/LZ_0.tex <==
$L_Z=1230_{-500}^{610}\,\mathrm{kpc\,km\,s^{-1}}$%


==> tex_text/LZ_2.tex <==
$L_Z=1200_{-640}^{710}\,\mathrm{kpc\,km\,s^{-1}}$%


==> tex_text/R_0.tex <==
$R=7.0_{-1.9}^{2.4}\,\mathrm{kpc}$%


==> tex_text/R_1.tex <==
$R=7.1_{-1.9}^{2.4}\,\mathrm{kpc}$%


==> tex_text/R_2.tex <==
$R=7.9_{-2.1}^{2.3}\,\mathrm{kpc}$%


==> tex_text/R_3.tex <==
$R=7.9_{-2.0}^{2.3}\,\mathrm{kpc}$%


==> tex_text/R_4.tex <==
$R=7.6_{-1.9}^{1.7}\,\mathrm{kpc}$%


==> tex_text/age_above_8gyr_below30perc_ageunc.tex <==
62\%%


==> tex_text/seq1_percentile_sigmas_sim_8.0_8.5.tex <==
0.050%


==> tex_text/seq1_percentile_sigmas_sim_8.5_9.0.tex <==
0.037%


==> tex_text/seq1_percentile_sigmas_sim_9.0_9.5.tex <==
0.037%


==> tex_text/seq1_percentiles_sim_all_8.5_9.0.tex <==
0.067%


==> tex_text/seq1_sigmas_sim_8.5_9.0.tex <==
0.043%


==> tex_text/seq2_mean_sigmas_sim_8.5_9.0.tex <==
$-0.652 \pm 0.020$%


==> tex_text/seq2_percentiles_sim_8.0_8.5.tex <==
$-0.632 \pm 0.016$%


==> tex_text/seq2_percentiles_sim_8.5_9.0.tex <==
$-0.653 \pm 0.012$%


==> tex_text/seq2_percentiles_sim_9.0_9.5.tex <==
$-0.681 \pm 0.028$%


==> tex_text/shift_by_4_to_5_gyr_median.tex <==
[C/H] by -0.27, [N/H] by -0.39, [O/H] by -0.26, [Ne/H] by -0.20, [Mg/H] by 0.17, [Al/H] by 0.08, [Si/H] by -0.34, [P/H] by -0.21, [S/H] by -0.29, [V/H] by -0.02, [Cr/H] by -0.19, [Mn/H] by -0.36, [Fe/H] by -0.15, [Co/H] by -0.03,  and [Ba/H] by -0.70%


==> tex_text/v_phi_sequence_3.tex <==
$V_\phi = 70_{-130}^{+160}\,\mathrm{kpc\,km\,s^{-1}}$%


==> tex_text/vphi_0.tex <==
$V_\phi=177.8_{-62.2}^{59.4}\,\mathrm{km\,s^{-1}}$%


==> tex_text/vphi_1.tex <==
$V_\phi=183.0_{-54.6}^{57.0}\,\mathrm{km\,s^{-1}}$%


==> tex_text/vphi_2.tex <==
$V_\phi=151.2_{-82.6}^{105.8}\,\mathrm{km\,s^{-1}}$%


==> tex_text/vphi_3.tex <==
$V_\phi=145.9_{-72.8}^{93.3}\,\mathrm{km\,s^{-1}}$%


==> tex_text/vphi_4.tex <==
$V_\phi=181.0_{-54.0}^{62.8}\,\mathrm{km\,s^{-1}}$%

